First Past the Post: Evaluating Query Optimization in MongoDB

Query optimization is crucial for every database management system (DBMS) to enable fast execution of declarative queries. Most DBMS designs include cost-based query optimization. However, MongoDB implements a different approach to choose an execution plan that we call "first past the post" (FPTP) query optimization. FPTP does not estimate costs for each execution plan, but rather partially executes the alternative plans in a round-robin race and observes the work done by each relative to the number of records returned. In this paper, we analyze the effectiveness of MongoDB's FPTP query optimizer. We see whether the optimizer chooses the best execution plan among the alternatives and measure how the chosen plan compares to the optimal plan. We also show how to visualize the effectiveness and identify situations where the MongoDB 7.0.1 query optimizer chooses suboptimal query plans. Through experiments, we conclude that FPTP has a preference bias, choosing index scans even in many cases where collection scans would run faster. We identify the reasons for the preference bias, which can lead MongoDB to choose a plan with more than twice the runtime compared to the optimal plan for the query.

==> 7-biographies.tex <==
\newcommand{\email}[1]{\href{mailto:#1}{#1}}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/people/dawei.jpeg}}]{Dawei Tao}
Dawei completed a Bachelor of Information Technology (Honours) in Computer Science at the University of Sydney. He is now a Graduate Software Engineer at Wilcom International.
\email{dtao7193@uni.sydney.edu.au}
\end{IEEEbiography}
\vspace{-1.5em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/people/enqi.jpeg}}]{Enqi Liu}
Enqi completed a Bachelor of Advanced Computing in Computational Data Science and Business Analytics at the University of Sydney.
\email{eliu5850@uni.sydney.edu.au}
\end{IEEEbiography}
\vspace{-1.5em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/people/harshana.jpeg}}]{Sidath Randeni Kadupitige}
Harshana completed a PhD in Genome Sciences / Genomics at the University of Sydney. He is now a Leading Teacher at UNSW College.
\email{sidath.randenikadupitige@sydney.edu.au}
\end{IEEEbiography}
\vspace{-1.5em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/people/michael.jpeg}}]{Michael Cahill}
Michael completed a PhD in Computer Science at the University of Sydney. After an industry career including as Vice President of Engineering at MongoDB, Michael is now a Professor of Practice in the School of Computer Science at the University of Sydney.
\email{michael.cahill@sydney.edu.au}
\end{IEEEbiography}
\vspace{-1.5em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/people/alan.jpeg}}]{Alan Fekete}
Alan is the Professor of Enterprise Software Systems at the University of Sydney. He carries out research in Database Transaction Management, with ongoing interest in Formal Methods and Computer Science Education.
\email{alan.fekete@sydney.edu.au}
\end{IEEEbiography}
\vspace{-1.5em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/people/uwe.jpeg}}]{Uwe R{\"o}hm}
Uwe is an Associate Professor in the School of Computer Science at the University of Sydney. His research areas include the integration of machine learning into database systems, data management on modern hardware, parallel query processing, and transaction processing with snapshot isolation.
\email{uwe.roehm@sydney.edu.au}
\end{IEEEbiography}

==> acknowledgement.tex <==
\begin{acks}
 This work was supported by the [...] Research Fund of [...] (Number [...]). Additional funding was provided by [...] and [...]. We also thank [...] for contributing [...].

 
 
 
\end{acks}

 
 

==> effect-of-caching.tex <==
\clearpage
\section{The effect of query plan cache}
Every query requires a query plan before it is actually executed. Whenever a query is run for the first time in MongoDB, a query plan is generated for the query. This query plan is cached with the shape of the query. In this way, when the queries with the same shape are run again, MongoDB reuses the cached query plan instead of creating a new one. 

Recall that query shape is essentially a query’s match expression, projection and sort with the values taken out. Therefore, all queries in the previous experiments have exactly the same query shape despite different query range. As a result, after the first query is executed, all other query statements will use its cached query plan. 

In this experiment, we aim at exploring the effect of query plan cache. Therefore, we simulated three cases where different query plan was cached first: 
\begin{enumerate}
    \item Plan A cached: An index scan on field A was cached first.
    \item Plan B cached: An index scan on field B was cached first.
    \item Plan C cached: A collection scan was cached first.
\end{enumerate}
As a result, all other queries will reuse the query plan of the first query that has been executed. We compared the execution time of the cached plan with that of the optimal plan (i.e. the query plan that has the shortest execution time). An impact factor is calculated based on averaging over plans from different selectivity.

\subsection{Without covering index}
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/plan_a_cached_mongo_choice.png}
    \caption{Plan A cached: MongoDB's chosen plans}
    \label{fig:a-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/plan_a_cached_practical_winner.png}
    \caption{Plan A cached: the optimal query plans}
    \label{fig:a-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-without-covering-index/mongo-original/plan_a_cached_summary_accuracy=24.92_overall_percentage_change=251.81.png}
    \caption{Plan A cached: MongoDB's chosen plans, accuracy = 24.92\%, impact factor = 251.81\%}
    \label{fig:a-cached-impact-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/plan_b_cached_mongo_choice.png}
    \caption{Plan B cached: MongoDB's chosen plans}
    \label{fig:b-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/plan_b_cached_practical_winner.png}
    \caption{Plan B cached: the optimal query plans}
    \label{fig:b-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-without-covering-index/mongo-original/plan_b_cached_summary_accuracy=27.60_overall_percentage_change=222.32.png}
    \caption{Plan B cached: MongoDB's chosen plans, accuracy = 27.60\%, impact factor = 222.32\%}
    \label{fig:b-cached-impact-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/plan_coll_cached_mongo_choice.png}
    \caption{Plan C cached: MongoDB's chosen plans}
    \label{fig:c-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/plan_coll_cached_practical_winner.png}
    \caption{Plan C cached: the optimal query plans}
    \label{fig:c-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-without-covering-index/mongo-original/plan_coll_cached_summary_accuracy=47.48_overall_percentage_change=198.12.png}
    \caption{Plan C cached: MongoDB's chosen plans, accuracy = 47.48\%, impact factor = 198.12\%}
    \label{fig:c-cached-impact-v0}
\end{figure}


\clearpage

==> extra-experiment.tex <==
\section{Extra experiments}
\textbf{Overview:} I would like to add following experiments to this article. We need to prioritize these sections and put them in right place.

\subsection{Task 1: Increase the diversity of the workload}
\noindent\textbf{Description: } The experiment in the thesis uses a very simple model. Although it is enough to demonstrate MongoDB's problem, we still need more complex datasets and queries to convince readers that the issue not only related to small datasets but also to datasets with more complex schema and index structure.\\ 

\noindent\textbf{Goal:} The final goal is to produce a plan diagram like the one Haritsa presented in his paper \url{https://dl.acm.org/doi/10.5555/1083592.1083735}, an example would be figure \ref{fig:plandiagram}. But the major difference is that we focus on the performance of the chosen plan instead of query plan cost.\\

\begin{figure}[tph]
    \centering
    \includegraphics[width=0.3\linewidth]{images/extra-experiments/plandiagram.png}
    \caption{Plan diagram}
    \label{fig:plandiagram}
\end{figure}

\noindent\textbf{My attempts: } 
I have checked how Haritsa produces that plan diagram. In the paper, he uses TCP-H workload. The query is a variation of query 7 of the TPC-H benchmark, with selectivity variations on the ORDERS and CUSTOMER relations. \\

\begin{verbatim}
// The original query 7 of the TPC-H benchmark
SELECT SUPP_NATION, CUST_NATION, L_YEAR, SUM(VOLUME) AS REVENUE
FROM ( SELECT N1.N_NAME AS SUPP_NATION, N2.N_NAME AS CUST_NATION, 
datepart(yy, L_SHIPDATE) AS L_YEAR,
 L_EXTENDEDPRICE*(1-L_DISCOUNT) AS VOLUME
 FROM SUPPLIER, LINEITEM, ORDERS, CUSTOMER, NATION N1, NATION N2
 WHERE S_SUPPKEY = L_SUPPKEY AND O_ORDERKEY = L_ORDERKEY AND C_CUSTKEY = O_CUSTKEY
 AND S_NATIONKEY = N1.N_NATIONKEY AND C_NATIONKEY = N2.N_NATIONKEY AND
 ((N1.N_NAME = 'FRANCE' AND N2.N_NAME = 'GERMANY') OR
 (N1.N_NAME = 'GERMANY' AND N2.N_NAME = 'FRANCE')) AND
 L_SHIPDATE BETWEEN '1995-01-01' AND '1996-12-31' ) AS SHIPPING
GROUP BY SUPP_NATION, CUST_NATION, L_YEAR
ORDER BY SUPP_NATION, CUST_NATION, L_YEAR
\end{verbatim}

The query above is a typical TPC-H query, involving various complex SQL operations, especially joins and subqueries. For a relational database, this query is very suitable to examine the effectiveness of the query optimizer. However, MongoDB is a NoSQL database, and it is non-relational. We cannot directly apply TPC-H benchmark. Here are two possible solutions:
1. Make MongoDB adapt to 
2. 


\subsection{Task 2: Investigate MongoDB Query Compiler and Optimizer(Done)}
\noindent\textbf{Description: } To understand how a MongoDB query is submitted, parsed and optimized before it interacts with MongoDB storage engine. See section 2.5.




==> figures-with-explanations.tex <==

\clearpage

\section{Figures With Explanations}

\subsection{Experiment results without covering index}


\noindent\textbf{Vanilla MongoDB}
\begin{enumerate}
    \item fig \ref{fig:mongo-choice-v0}
    \item fig \ref{fig:mongo-with-coll-v0}
    \item fig \ref{fig:mongo-with-fix-v0}
\end{enumerate}

\noindent\textbf{MongoDB with collection scan but failed to choose collection scan}
\begin{enumerate}
    \item fig \ref{fig:mongo-choice-v1}
    \item fig \ref{fig:mongo-with-coll-v1}
    \item fig \ref{fig:mongo-with-fix-v1}
\end{enumerate}


\noindent\textbf{MongoDB with fix}
\begin{enumerate}
    \item fig \ref{fig:mongo-choice-v2}
    \item fig \ref{fig:mongo-with-coll-v2}
    \item fig \ref{fig:mongo-with-fix-v2}
\end{enumerate}



\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/comprehensive_mongo_choice.png}
    \caption{A visualization of chosen plans}
    \label{fig:mongo-choice-v0}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-original/comprehensive_practical_winner.png}
    \caption{A visualization of optimal plans in terms of execution time}
    \label{fig:mongo-with-coll-v0}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-without-covering-index/mongo-original/comprehensive_summary_accuracy=51.96_overall_percentage_change=26.23.png}
    \caption{A visualization of impact. Accuracy = 51.96\%, Performance diff = 26.23\%}
    \label{fig:mongo-with-fix-v0}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-with-coll/comprehensive_mongo_choice.png}
    \caption{A visualization of chosen plans}
    \label{fig:mongo-choice-v1}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-with-coll/comprehensive_practical_winner.png}
    \caption{A visualization of optimal plans in terms of execution time}
    \label{fig:mongo-with-coll-v1}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-without-covering-index/mongo-with-coll/comprehensive_summary_accuracy=55.76_overall_percentage_change=20.34.png}
    \caption{A visualization of impact. Accuracy = 55.76\%, Performance diff = 20.34\%}
    \label{fig:mongo-with-fix-v1}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-with-coll-with-fix/comprehensive_mongo_choice.png}
    \caption{A visualization of chosen plans}
    \label{fig:mongo-choice-v2}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-without-covering-index/mongo-with-coll-with-fix/comprehensive_practical_winner.png}
    \caption{A visualization of optimal plans in terms of execution time}
    \label{fig:mongo-with-coll-v2}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-without-covering-index/mongo-with-coll-with-fix/comprehensive_summary_accuracy=85.12_overall_percentage_change=2.09.png}
    \caption{A visualization of impact. Accuracy = 85.12\%, Performance diff = 2.09\%}
    \label{fig:mongo-with-fix-v2}
\end{figure}






\subsection{Experiments with query plan cache enabled}

\noindent\textbf{An index scan on A is cached}
\begin{enumerate}
    \item fig \ref{fig:cover-a-cached-v0}
    \item fig \ref{fig:cover-a-cached-optimal-v0}
    \item fig \ref{fig:cover-a-cached-impact-v0}
\end{enumerate}

\noindent\textbf{An index scan on B is cached}
\begin{enumerate}
    \item fig \ref{fig:cover-b-cached-v0}
    \item fig \ref{fig:cover-b-cached-optimal-v0}
    \item fig \ref{fig:cover-b-cached-impact-v0}
\end{enumerate}

\noindent\textbf{A covering index is cached}
\begin{enumerate}
    \item fig \ref{fig:cover-cover-cached-v0}
    \item fig \ref{fig:cover-cover-cached-optimal-v0}
    \item fig \ref{fig:cover-cover-cached-impact-v0}
\end{enumerate}

\noindent\textbf{A collection scan is cached}
\begin{enumerate}
    \item fig \ref{fig:cover-coll-cached-v0}
    \item fig \ref{fig:cover-coll-cached-optimal-v0}
    \item fig \ref{fig:cover-coll-cached-impact-v0}
\end{enumerate}




\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_a_cached_mongo_choice.png}
    \caption{Plan A cached: MongoDB's chosen plans}
    \label{fig:cover-a-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_a_cached_practical_winner.png}
    \caption{Plan A cached: the optimal query plans}
    \label{fig:cover-a-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-with-covering-index/mongo-original/plan_a_cached_summary_accuracy=0.00_overall_percentage_change=341.30.png}
    \caption{Plan A cached: MongoDB's chosen plans, accuracy = 0.00\%, impact factor = 341.30\%}
    \label{fig:cover-a-cached-impact-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_b_cached_mongo_choice.png}
    \caption{Plan B cached: MongoDB's chosen plans}
    \label{fig:cover-b-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_b_cached_practical_winner.png}
    \caption{Plan B cached: the optimal query plans}
    \label{fig:cover-b-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-with-covering-index/mongo-original/plan_b_cached_summary_accuracy=20.68_overall_percentage_change=673.99.png}
    \caption{Plan B cached: MongoDB's chosen plans, accuracy = 20.68\%, impact factor = 673.99\%}
    \label{fig:cover-b-cached-impact-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_coll_cached_mongo_choice.png}
    \caption{Plan coll cached: MongoDB's chosen plans}
    \label{fig:cover-coll-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_coll_cached_practical_winner.png}
    \caption{Plan coll cached: the optimal query plans}
    \label{fig:cover-coll-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-with-covering-index/mongo-original/plan_coll_cached_summary_accuracy=5.24_overall_percentage_change=365.99.png}
    \caption{Plan coll cached: MongoDB's chosen plans, accuracy = 5.24\%, impact factor = 365.99\%}
    \label{fig:cover-coll-cached-impact-v0}
\end{figure}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_cover_cached_mongo_choice.png}
    \caption{Plan cover cached: MongoDB's chosen plans}
    \label{fig:cover-cover-cached-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{images/results-with-covering-index/mongo-original/plan_cover_cached_practical_winner.png}
    \caption{Plan cover cached: the optimal query plans}
    \label{fig:cover-cover-cached-optimal-v0}
\end{figure}


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\linewidth]{images/results-with-covering-index/mongo-original/plan_cover_cached_summary_accuracy=74.08_overall_percentage_change=96.12.png}
    \caption{Plan cover cached: MongoDB's chosen plans, accuracy = 74.08\%, impact factor = 96.12\%}
    \label{fig:cover-cover-cached-impact-v0}
\end{figure}
